One ISAC Array, Two Worst Cases: Hardware Impairments in Beamforming and AoA Estimation

In integrated sensing and communication (ISAC), the same base-station array beamforms toward users and estimates their angle of arrival (AoA). In this paper, we study how element-level gain, phase, and position errors affect both functions of a beam-scanning uniform linear array. Any array produces a correlation peak at the true angle, of finite height and width, surrounded by sidelobes. Impairments shift this peak, make it lower and wider, and raise the sidelobes relative to it. A single decomposition explains these three effects: the gain-weighted least-squares fit of the per-antenna phase errors splits them into a tilt, which shifts the peak, and a residual, whose power is taken from the peak and redistributed over the sidelobes according to its spatial spectrum. A beam steered toward the strongest direction suffers from the lower peak only, whereas the AoA estimate suffers from its shift even without noise, and also from the lowering and sidelobes with noise. The worst cases for the two ISAC functions are thus nearly disjoint, and we characterize both: the worst case for beamforming leaves the AoA estimate unbiased, and the worst case for localization loses little beamforming gain. The worst case for localization is a single defect at the junction between two subarrays, and its error, relative to the main-lobe width, does not decrease with the number of antennas. We also characterize random impairments and the effect of noise. In practical terms, our analysis shows that the calibration of a dual-function array must be assessed with respect to both functions.

==> fig_decomposition_tikz.tex <==
%% Illustration of the tilt and residual decomposition of the phase errors (N = 8, random impairments).
%% Requires: \usepackage{tikz}  \usetikzlibrary{arrows.meta,calc}
\begin{tikzpicture}[font=\footnotesize, x=1.75cm, y=0.032cm]
  \colorlet{tiltc}{orange!85!black}\colorlet{resc}{blue!60!black}
  \draw[-{Triangle[length=1.6mm, width=1.3mm]}, black!70] (-2.05,0) -- (2.15,0) node[below left, font=\scriptsize] {$d_k-\bar d$};
  \draw[-{Triangle[length=1.6mm, width=1.3mm]}, black!70] (-2.05,-62) -- (-2.05,66) node[right, font=\scriptsize] {$\Psi_k$ (deg)};
  \foreach \y in {-50,50} { \draw[black!60] (-2.08,\y) -- (-2.02,\y) node[left=1pt, font=\tiny] {$\y$}; }
  \foreach \x in {-1.5,-1,-0.5,0.5,1,1.5} { \draw[black!60] (\x,-2) -- (\x,2); }
  \node[below, font=\tiny] at (1,-2) {$1$}; \node[below, font=\tiny] at (-1,-2) {$-1$};
  %% tilt: gain-weighted least-squares line
  \draw[tiltc, line width=1.1pt] (-1.95,-27.15) -- (1.95,51.09);
  %% residuals and antennas (marker size = gain)
  \foreach \xx/\yy/\g/\yl in {-1.695/-57.02/0.891/-22.04, -1.195/13.91/0.515/-12.01, -0.695/-3.10/0.569/-1.98, -0.195/47.28/0.807/8.05, 0.305/22.75/0.935/18.08, 0.805/36.51/0.784/28.11, 1.305/15.66/0.518/38.15, 1.805/27.43/0.603/48.18} {
    \draw[resc, line width=0.8pt] (\xx,\yl) -- (\xx,\yy);
    \fill[resc] (\xx,\yy) circle[radius={(0.9+1.6*\g)*1pt}];
  }
  \node[tiltc, anchor=south west, font=\scriptsize] at (0.55,61.09) {tilt: slope $2\pi\Delta_0^\star$};
  \node[resc, anchor=north west, font=\scriptsize, align=left] at (-1.95,-30) {residual $r_k$\\[-1pt](vertical segments)};
\end{tikzpicture}

